A Hybrid Partitioning Strategy for Backward Reachability of Neural Feedback Loops

As neural networks become more integrated into the systems that we depend on for transportation, medicine, and security, it becomes increasingly important that we develop methods to analyze their behavior to ensure that they are safe to use within these contexts. The methods used in this paper seek to certify safety for closed-loop systems with neural network controllers, i.e., neural feedback loops, using backward reachability analysis. Namely, we calculate backprojection (BP) set over-approximations (BPOAs), i.e., sets of states that lead to a given target set that bounds dangerous regions of the state space. The system's safety can then be certified by checking its current state against the BPOAs. While over-approximating BPs is significantly faster than calculating exact BP sets, solving the relaxed problem leads to conservativeness. To combat conservativeness, partitioning strategies can be used to split the problem into a set of sub-problems, each less conservative than the unpartitioned problem. We introduce a hybrid partitioning method that uses both target set partitioning (TSP) and backreachable set partitioning (BRSP) to overcome a lower bound on estimation error that is present when using BRSP. Numerical results demonstrate a near order-of-magnitude reduction in estimation error compared to BRSP or TSP given the same computation time.

==> related_work.tex <==
%!TEX root=main.tex

\section{Related Work}

Open-loop NN analysis, i.e., the determination of a set of possible NN outputs given a set of inputs \cite{}, is a growing field of research motivated by a desire for safety from adversarial attacks \cite{}.
These tools generally exist on a spectrum from fast but conservative \cite{} to slow but exact \cite{}.
Analysis of closed-loop systems for the purpose of safety certification has historically consisted of forward reachability analysis \cite{bansal2017hamilton, evans1998partial}, i.e., determining a set of possible future states from a set of initial states, and backward reachability analysis \cite{xue2016under, kochdumper2020computing, yang2021scalable}, i.e., determining a set of previous states that lead to a set of final target states.
To combine open-loop NN analysis and closed-loop analysis techniques, recent work has led to the development of methods for forward \cite{dutta2019reachability, huang2019reachnn, ivanov2019verisig, fan2020reachnn, xiang2020reachable, hu2020reach, sidrane2021overt, everett2021reachability, vincent2021reachable} and backward reachability analysis \cite{bak2022closed, rober2022backward, rober2022partition, vincent2021reachable} for NFLs.

This work focuses on a backward reachability method developed in \cite{rober2022backward, rober2022partition}, motivated by the discussion therein.
Specifically, because \cite{rober2022partition} uses CROWN \cite{zhang2018efficient}, which falls on the "fast but conservative" end of the open-loop NN analysis spectrum, we investigate partitioning strategies with the goal of reducing conservativeness in the NN relaxation, resulting in lower approximation error in the BPOAs.
While backward reachability partitioning techniques were introduced in \cite{rober2022partition}, it was noted that they had a fundamental limitation causing a lower bound on the approximation error.
Partitioning has also been studied for forward reachability of NFLs, with \cite{everett2021efficient} 
Ref \cite{everett2021efficient, others} use partitioning techniques wherein the initial state set is split into smaller partitions and the forward reachability problem is solved for each.






% Reachability analysis can be broadly categorized into three categories by system type: NNs in isolation (i.e., open-loop analysis), closed-loop systems without neural components, and NFLs.

% Open-loop NN analysis encompasses techniques that relax the nonlinearities in the NN activation functions to quickly provide relatively conservative bounds on NN outputs~\cite{zhang2018efficient, raghunathan2018semidefinite}, and techniques that take more time to provide exact bounds~\cite{katz2017reluplex, vincent2021reachable}.
% % Generally, these techniques exist on a spectrum from exact but slow~\cite{katz2017reluplex, vincent2021reachable} to conservative but fast~\cite{zhang2018efficient, raghunathan2018semidefinite}.
% % Typically, these analyses are conducted on the NN in isolation, often focusing on guaranteeing robustness to adversarial attacks against perception models~\cite{raghunathan2018semidefinite, tjeng2017evaluating}. 
% % However, when considering NNs and their relationship to autonomous systems, it is often desirable to provide analysis of the entire closed-loop system. 
% Many of these open-loop studies are motivated by the goal of guaranteeing robustness to adversarial attacks against perception models~\cite{raghunathan2018semidefinite, tjeng2017evaluating}, but cannot be directly used to guarantee safety for closed-loop systems because they do not consider closed-loop system dynamics.

% % In contrast to open-loop analysis, NFL analysis tools seek to answer questions about complete closed-loop systems. The majority of work in this area is centered on forward reachability analysis~\cite{dutta2019reachability, huang2019reachnn, ivanov2019verisig, fan2020reachnn, xiang2020reachable, hu2020reach, sidrane2021overt, everett2021reachability}.

% For closed-loop systems without NNs, reachability analysis is a well established method of providing safety verification.
% Hamilton-Jacobi methods~\cite{bansal2017hamilton, evans1998partial}, CORA~\cite{althoff2015introduction}, Flow*~\cite{chen2013flow}, SpaceEx~\cite{frehse2011spaceex}, HYLAA~\cite{bak2017hylaa}, and C2E2~\cite{duggirala2015c2e2} are tools that are commonly used for reachability analysis, but because they do not handle open loop NN analysis, they cannot be used to analyze NFLs.

% % Many studies have developed techniques for forward reachability analysis of NFLs~\cite{dutta2019reachability, huang2019reachnn, ivanov2019verisig, fan2020reachnn, xiang2020reachable, hu2020reach, sidrane2021overt, everett2021reachability}, but unlike traditional systems where a simple change of variables can be used to switch from forward to backward reachability ~\cite{bansal2017hamilton,evans1998partial}, backward reachability analysis is particularly challenging when NNs are involved. 
% % In particular, a key challenge with propagating sets backward through NNs is that common NN activations have finite range (e.g., $\mathrm{ReLU}(x) = 0$ could correspond to any $x \leq 0$), which causes the sets to quickly explode to an infinite range of possible inputs.
% % Moreover, even when using an infinite range activation (e.g., Leaky ReLU), the NN's weight matrices may not be invertible (e.g., singular, rank deficient).
% % Recent work related to NN inversion has developed specific invertible-by-design NN architectures~\cite{ardizzone2018analyzing} and modifications to the training procedure to regularize for invertibility~\cite{behrmann2019invertible}.
% % In contrast to strategies that depend on invertibility to propagate sets backward through a NN, our approach can be applied to any NN for which an affine relaxation can be computed, i.e., the same broad class of NN architectures (e.g., feedforward NNs with general activation functions) with arbitrary training processes that CROWN (or recent extensions~\cite{xu2020automatic,xu2021fast,wang2021beta}) operates on.

% Forward reachability analysis is the focus of many recent works~\cite{dutta2019reachability, huang2019reachnn, ivanov2019verisig, fan2020reachnn, xiang2020reachable, hu2020reach, sidrane2021overt, everett2021reachability}, but while more traditional approaches to reachability analysis, e.g., Hamilton-Jacobi methods, can easily switch from forward to backward with a change of variables~\cite{bansal2017hamilton, evans1998partial}, backward reachability for NFLs is less straightforward.
% One challenge with propagating sets backward through a NN is that many activation functions have finite range, meaning that there is not a one-to-one mapping of inputs to outputs (e.g., $\mathrm{ReLU}(x) = 0$ corresponds to all values of $x \leq 0$), which can cause large amounts of conservativeness in the BP set estimate as there is an infinite set of possible inputs.
% Additionally, even if an infinite-range activation function is used, NN weight matrices may be singular or rank deficient and are thus generally not invertible, again causing problems with determining inputs given a set of outputs.
% While recent works on NN inversion have developed NN architectures that are designed to be invertible~\cite{ardizzone2018analyzing} and training procedures that regularize for invertibility~\cite{behrmann2019invertible}, dependence on these techniques would be a major limitation on the class of systems for which backward reachability analysis could be applied.
% Our approach avoids the challenges associated with finite-range activation functions and NN-invertibility and can be applied to the same class of NN architectures as CROWN \cite{zhang2018efficient}, i.e. NNs for which an affine relaxation can be found.

% % While the body of work concerning reachability analysis is growing, less attention has been paid to the reverse problem of finding \emph{backprojection} sets, i.e. the set of possible states for which the NN control policy will deliver the system to a target set. 
% Several recent works have investigated backwards reachability analysis for NFLs.
% Ref.~\cite{vincent2021reachable} describes a method for open-loop backward reachability on a NN dynamics model, but this method does not directly apply to this work's problem of interest, namely a NN controller with known dynamics.
% % but they do not extend their results to closed-loop systems, and to do so with their methods would be computationally expensive.
% Alternatively, while~\cite{bak2022closed} analyzes NFLs, they use a quantized state approach~\cite{jia2021verifying} that requires an alteration of the original NN through a preprocessing step that can affect its overall behavior.
% Finally, previous work by the authors~\cite{everett2021reachability} derives a closed-form equation that can be used to find under-approximations of the BP set, but this is most useful for goal checking when it is desirable to guarantee that all states in the BP estimate will reach the target set.
% This work builds off of~\cite{everett2021reachability}, adapting some of the steps used to find BP under-approximations to instead find BP over-approximations, which are good for obstacle avoidance because they contain all the states that reach the target set.

% \iffalse
% % TODO: work this into the discussion
% Recent related work has developed specific invertible-by-design NN architectures~\cite{ardizzone2018analyzing} and modifications to the training procedure to regularize for invertibility~\cite{behrmann2019invertible}.
% In contrast, our approach can be applied to any NN for which an affine relaxation can be computed, i.e., the same broad class of NN architectures (e.g., feedforward NNs with general activation functions) with arbitrary training processes that CROWN (or recent extensions~\cite{xu2020automatic,xu2021fast,wang2021beta}) operates on.

% % TODO: work this into the discussion
% Recall that converting a reachability analysis method from forward to backward is particularly challenging when NNs are involved, as opposed to the straightforward change of variables for systems without NN components~\cite{bansal2017hamilton,evans1998partial}.
% In particular, a key challenge with propagating sets \textit{backward} through NNs is that common NN activations have finite range (e.g., $\mathrm{ReLU}(x) = 0$ could correspond to any $x \leq 0$), which causes the sets to quickly explode to $\infty$.
% Moreover, even using an infinite range activation (e.g., Leaky ReLU), the weight matrices may not be invertible (e.g., singular, insufficient rank).
% Our approach is able to avoid these issues and still leverage forward propagation tools (e.g., CROWN~\cite{zhang2018efficient}) despite thinking backward in time.
% \fi
